A Computational Framework for Behavioral Assessment of LLM Therapists

The emergence of large language models (LLMs) like ChatGPT has increased interest in their use as therapists to address mental health challenges and the widespread lack of access to care. However, experts have emphasized the critical need for systematic evaluation of LLM-based mental health interventions to accurately assess their capabilities and limitations. Here, we propose BOLT, a proof-of-concept computational framework to systematically assess the conversational behavior of LLM therapists. We quantitatively measure LLM behavior across 13 psychotherapeutic approaches with in-context learning methods. Then, we compare the behavior of LLMs against high- and low-quality human therapy. Our analysis based on Motivational Interviewing therapy reveals that LLMs often resemble behaviors more commonly exhibited in low-quality therapy rather than high-quality therapy, such as offering a higher degree of problem-solving advice when clients share emotions. However, unlike low-quality therapy, LLMs reflect significantly more upon clients' needs and strengths. Our findings caution that LLM therapists still require further research for consistent, high-quality care.

==> images/fig-10-simulation-full-real-example.tex <==
\begin{figure*}[t]
\caption{Illustration on the Full Response Simulation Method with Real Example \tim{does real mean "in fact generated by one of our  models"? clariy and specify model} \tim{i love that you're adding these examples - I  even wonder  whether we should integrate one in the  main paper. However, I ddon't understand how to read tihs figure. what are the a/b. What is round one/two. Can you simplify and/or explain  more  clearly how to read this?}}
\includegraphics[width=0.8\textwidth]{images/LLM_simulation_image_full.pdf}
\centering
\label{fig:simulation_Full_response_illustration}
\end{figure*}

==> images/fig-2-distribution.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth]{images/distribution_hl.pdf}
\centering
\vspace{-20pt}
\caption{Difference in the \textit{frequency} of conversational behaviors exhibited by LLM therapists (GPT-4, GPT-3.5-turbo, Llama2-70b, Llama2-13b) or low-quality human therapy, relative to high-quality human therapy. Values $>0\%$ (colored in \textcolor{blueplot}{blue}) indicate significantly higher frequency whereas values $<0\%$ (colored in \textcolor{orangeplot}{orange}) indicate significantly lower frequency of a particular behavior as compared to high-quality human therapy. Values in \textcolor{gray}{gray} are not statistically significantly different from zero at p = 0.05 using Two-sided Student’s t-test. Error bars indicate 95\% bootstrapped confidence intervals. For instance, GPT-4 responds with $28.20\%$ more \textsc{Problem-Solving} than high-quality human therapy (Cohen's $h = \num{0.62}$, $P = \num{1.8E-248}$, $t = 33.67$; d.f. $= 3726$, two-sided Student’s $t$-test). A key insight we find is that all LLMs respond with significantly higher \textsc{Problem-Solving}, similar to low-quality human therapy.}
\vspace{-10pt}

\label{fig:distribution-avg}
\end{figure*}

==> images/fig-2-new-analysis-overview.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{images/New-Analysis-Overview.pdf}
\centering
% \vspace{-25pt}
\caption{Overview of our analysis approach. We establish a baseline by calculating the average conversational behavior across all human therapy conversations. We consider behaviors aligned with low-quality conversations as below average quality and behaviors aligned with high-quality conversations as above average quality. We then assess the LLM therapists' behavior in relation to this average. This allows us to assess whether the behavior of LLM therapists falls below or above this average, indicating closer alignment with low-quality or high-quality human therapists, respectively. In this example figure, the behaviors of LLM A and LLM B is potentially undesirable because they are below average quality and closer to low-quality therapy than high-quality therapy. The behavior of LLM C is potentially desirable as it is closer to high-quality therapy. The behavior of LLM D is more than two standard deviations away from high-quality therapy which is why it is uncertain whether such behavior is desirable.    }
\label{fig:analysis-overview}
\end{figure*}

==> images/fig-3-first-occurence.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth]{images/firstorder_hl.pdf}
\centering
\vspace{-10pt}

\caption{Difference in the \textit{temporal order} of conversational behaviors, operationalized as the turn numbers in which behaviors are first exhibited in a conversation by LLM therapists (GPT-4, GPT-3.5-turbo, Llama2-70b, Llama2-13b) or low-quality human therapy, relative to high-quality human therapy. Values $>0$ (highlighted in \textcolor{blueplot}{blue}) indicate that the behavior is first expressed at a later turn whereas Values $<0$ (highlighted in \textcolor{orangeplot}{orange}) indicate that the behavior is first expressed earlier as compared to high-quality human therapy. Values in \textcolor{gray}{gray} are not statistically significantly different from zero at p = 0.05 using Two-sided Student’s t-test. Error bars indicate 95\% bootstrapped confidence intervals. For instance, GPT-4 first responds with \textsc{Planning} $5.04$ turns earlier than human high-quality therapy (Cohen's $d = \num{-2.02}$, $P = \num{7.4E-5}$, $t = -4.00$; d.f. $= 526$, two-sided Student’s $t$-test). Most LLM therapists start providing \textsc{Solutions} earlier in the conversations, but providing \textsc{Reflections on} client problems later against common recommendations \cite{cochran2015heart}.} 
\vspace{-10pt}
\label{fig:first_occur_avg}
\end{figure*}

==> images/fig-4-relative-occurence.tex <==
\begin{figure}[h]
\caption{Difference in the temporal order of conversational behaviors exhibited for all occurrences during a conversation by LLM therapists (GPT-4, GPT-3.5-turbo, Llama2-70b, Llama2-13b) or low-quality human therapy and high-quality human therapy. Values $>0\%$ (highlighted in \textcolor{blueplot}{blue}) indicate that a particular behavior is expressed at a significantly later stage whereas values $<0\%$ (highlighted in \textcolor{orangeplot}{orange}) indicate particular behavior is expressed at a significantly earlier stage as compared to high-quality human therapy. Values in \textcolor{gray}{gray} are not statistically significantly different from zero at p = 0.05 using Two-sided Student’s t-test. For instance, GPT-4 responds with \textsc{Problem-Solving} 2.29 turns earlier than human high-quality therapy (Cohen's $d = \num{-2.31}$, $P = \num{1.3E-7}$, $t = -5.29$; d.f. $= 2558$, two-sided Student’s $t$-test). In general, the trend presented here is similar to the first occurrences graph, for instance, LLM therapists tend to give more \textsc{Questions} similar to low-quality therapy.}
\includegraphics[width=\textwidth]{images/relativeorder_hl.pdf}
\label{fig:relative_occur_avg}
\end{figure}


==> images/fig-5-client-vs-therapist.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth]{images/client_vs_therapist_hl.pdf}
\centering
\vspace{-15pt}
\caption{Difference between the frequency of conversational behaviors observed in LLM therapists (GPT-4, GPT-3.5-turbo, Llama2-70b, Llama2-13b) or low-quality human therapy \textit{in response to specific client behaviors} (\textit{Adaptability}), relative to the frequency of behavior observed in high-quality human therapy in the same case.
% the frequency of the behavior observed in high-quality human therapy in response to different client behaviors. 
Values $>0\%$ (colored in \textcolor{blueplot}{blue}) indicate significantly higher frequency whereas values $<0\%$ (colored in \textcolor{orangeplot}{orange}) indicate significantly lower frequency as compared to high-quality human therapy.
Values in \textcolor{gray}{gray} are not statistically significantly different from zero at p = 0.05 using Two-sided Student’s t-test. Error bars indicate 95\% bootstrapped confidence intervals. For instance, GPT-4 exhibits $8.8\%$ more \textsc{Psychoeducation} than high-quality human therapy when the client expresses \textsc{Gained Insights} (Cohen's $h = \num{6.41}$, $P = \num{1.2E-3}$, $t = 3.24$; d.f. $= 16$, two-sided Student’s $t$-test). Here, one finding is that all LLMs respond with relatively higher \textsc{Psychoeducation} when compared with high-quality human therapy if the client expresses \textsc{Gained Insights}, similar to low-quality human therapy. }
\label{fig:client-vs-therapist_avg}
\end{figure*}


==> images/fig-9-simulation-single-real-example.tex <==
\begin{figure*}[t]
\caption{Illustration on the Single Response Simulation Method with Real Example.}
\includegraphics[width=0.8\textwidth]{images/LLM_simulation_image_single.pdf}
\centering
\label{fig:simulation_single_response_illustration}
\end{figure*}

==> images/fig-liwc.tex <==
\begin{figure*}
% \includegraphics[width=\textwidth]{images/liwc_analysis.pdf}
\centering
\vspace{-20pt}
\caption{\kelly{need to add the results}Difference between the word usage of LIWC categories in LLM therapists i(GPT-4, GPT-3.5-turbo, Llama2-70b, Llama2-13b), relative to average-, low-, and high-quality human therapy. \textbf{A}: average-quality, Low: low-quality, and High: high-quality therapy. The direction of the arrow on the x-axis indicates the direction in which the order is increasing (we flip the axis if low-quality is exhibited later than high-quality, such that low-quality is visualized below the average quality marker). Values colored in \textcolor{blueplot}{blue} indicate desirable behaviors (significantly closer to high-quality than low-quality) whereas values colored in \textcolor{orangeplot}{orange} indicate undesirable behaviors (significantly closer to low-quality than high-quality). Values in \textcolor{purpleplot}{purple} are two standard deviations above high-quality therapy and therefore it is uncertain whether they are potentially desirable. Values in \textcolor{gray}{gray} are not statistically significantly different from average-quality at p = 0.05 using Two-sided Student’s t-test. Error bars indicate 95\% bootstrapped confidence intervals. }

\end{figure*}



==> tables/table-10-therapist-classification-performance-per-intent.tex <==
\begin{table*}[t]
    \centering
    \small
        \caption{Therapist Conversational Behavior Classification Model Performance Details. We examine the performance of our model across different classes. See the result description in Methods.}
    % \resizebox{0.5\textwidth}{!}{%
    \def\arraystretch{1.15}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|cc}
         \toprule %\\[5pt]
         \multirow{2}{*}{\textbf{Behavior}} & \multicolumn{2}{c}{\textbf{Therapist}} \\
         \cmidrule(lr){2-3}
        & \multicolumn{1}{c}{\textbf{Macro F1}} & \multicolumn{1}{c}{\textbf{Accuracy}} \\
         \midrule
 \multicolumn{3}{c}{\textsc{\textbf{Reflections on}}} \\
 \midrule
 \textsc{Needs}  &  $72.8_{3.5}$&  $85.2_{4.6}$\\
 \midrule
 \textsc{Emotions}  &  $68_{4.1}$&  $88.2_{2.1}$\\
 \midrule
 \textsc{Values}&  $64.9_{8.1}$&  $91.3_{2.9}$\\
 \midrule
 \textsc{Consequences} &  $56.2_{12.6}$&  $91.6_{1.9}$\\
 \midrule
 \textsc{Conflict}  &  $54.5_{13.7}$&  $94.1_{1.6}$\\
 \midrule
 \textsc{Strength} &  $54.3_{13.7}$&  $88.7_{1.3}$\\
 \midrule
\multicolumn{3}{c}{\textsc{\textbf{Questions on}}} \\
\midrule
 \textsc{Experiences} &  $53.9_{16.2}$&  $75.6_{2.3}$\\
  \midrule
 \textsc{Perspectives} &  $53.8_{12.9}$&  $91.1_{1.1}$\\
  \midrule
 \textsc{Emotions}&  $47.7_{9.6}$&  $95.3_{1.5}$\\
 \midrule
\multicolumn{3}{c}{\textsc{\textbf{Solutions}}} \\
\midrule
 \textsc{Problem-Solving} &  $45.4_{7.1}$&  $87.4_{1.4}$\\
  \midrule
 \textsc{Planning}&  $42.6_{3.9}$&  $82.1_{2.4}$\\
 \midrule
 \multicolumn{3}{c}{\textsc{\textbf{Normalizing}}} \\
 \midrule
 \textsc{Normalizing} &  $41.0_{6.2}$&  $87.7_{1.7}$\\
 \midrule
 \multicolumn{3}{c}{\textsc{\textbf{Psychoeducation}}} \\
 \midrule
 \textsc{Psychoeducation} &  $35.3_{7.9}$&  $94.8_{1.0}$\\
    \bottomrule
    \end{tabular}
     \label{tab:therapist_individual_performance}
\end{table*}




==> tables/table-11-client-classification-performance-per-intent.tex <==
\begin{table*}[t]
    \centering
    \small
        \caption{Client Conversational Behavior Classification Model Performance Details. We examine the performance of our model across different classes. See the result description in Methods.}
    % \resizebox{0.7\textwidth}{!}{%
    \def\arraystretch{1.15}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|cc}
         \toprule %\\[5pt]
         \multirow{2}{*}{\textbf{Behavior}} & \multicolumn{2}{c}{\textbf{Client}} \\
         \cmidrule(lr){2-3}
        & \multicolumn{1}{c}{\textbf{Macro F1}} & \multicolumn{1}{c}{\textbf{Accuracy}} \\

 \midrule
 \textsc{Changing unhealthy behavior} & $65.1_{14.2}$ & $86.6_{5.0}$\\
 \midrule
 \textsc{Sustaining unhealthy behavior}  & $86.0_{11.6}$ & $95.4_{4.0}$\\
 \midrule
 \textsc{Sharing negative feeling or emotion} & $78.8_{4.4}$ & $81.0_{4.4}$\\
 \midrule
 \textsc{Sharing positive feeling or emotion} & $75.0_{9.5}$ & $92.8_{3.5}$\\
 \midrule
 \textsc{Gained Insight}& $66.9_{14.1}$ & $93.3_{3.0}$\\
 \midrule
 \textsc{Sharing Experiences} & $62.5_{15.1}$ & $82.9_{5.7}$\\
    \bottomrule
    \end{tabular}
    % }
    \label{tab:client_individual_performance}
    % \vspace{-10pt}
\end{table*}


==> tables/table-3-high-low-distribution.tex <==
\begin{table*}[t]
    \centering
    \small
    \caption{Difference between the frequency of conversational behaviors observed in LLM therapists (GPT-4, GPT-3.5-turbo, Llama2-70b, Llama2-13b) or low-quality human therapists and the frequency of the behavior observed in high-quality human therapists based on the two conversation simulation methods (single response and full conversation) on the High-Low Quality dataset from \cite{perez-rosas-etal-2019-makes}. We report the average percentage differences across the simulated conversations with standard deviations as subscripts. Positive values indicate significantly higher observed frequency of a particular behavior whereas negative values indicate significantly lower observed frequency of a particular behavior as compared to high-quality human therapists. Values in \textcolor{gray}{gray} are not statistically significant at p = 0.05 using a Two-sided Student's t-test.
 For instance, GPT-4 with single response simulation method has exhibited $16.27\%$ more \textsc{Reflection on Needs} behavior than high-quality human therapy.}
    \resizebox{1.01\textwidth}{!}{%
    \def\arraystretch{1.15}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|ccccccccc}
         \toprule %\\[5pt]
         \multirow{2}{*}{\textbf{Behavior}} & \multicolumn{4}{c}{\textbf{LLM Single Response}} & \multicolumn{4}{c}{\textbf{LLM Full Conversation}} & \textbf{Human} \\
         \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule{10-10}
        & GPT-4 & GPT-3.5 & Llama2-70b & Llama2-13b  & GPT-4 & GPT-3.5 & Llama2-70b & Llama2-13b & Low-Quality \\
         \midrule
 \multicolumn{10}{c}{\textsc{\textbf{Reflections on}}} \\
 \midrule
 \textsc{Needs} &$\phantom{-}16.27^*_{\pm  2.08}$&$\phantom{-}5.40^*_{\pm  2.01}$&$\phantom{-}13.96^*_{\pm  2.06}$&$\phantom{-}11.79^*_{\pm  2.05}$&$\phantom{-}4.88^*_{\pm  3.11}$&$\phantom{-}9.22^*_{\pm  3.51}$&$-5.41^*_{\pm  2.80}$&$-6.29^*_{\pm  2.92}$&$-5.59^*_{\pm  2.45}$\\
 \textsc{Emotions} &$\phantom{-}\textcolor{gray}{0.71^{\phantom{*}}_{\pm  1.59 }}$&$\phantom{-}7.12^*_{\pm  1.70}$&$\phantom{-}1.74^*_{\pm  1.60}$&$\phantom{-}\textcolor{gray}{0.89^{\phantom{*}}_{\pm  1.59 }}$&$-6.19^*_{\pm  2.01}$&$-6.15^*_{\pm  2.19}$&$-5.31^*_{\pm  2.07}$&$-4.78^*_{\pm  2.22}$&$-8.31^*_{\pm  1.65}$ \\
 \textsc{Values} &$\textcolor{gray}{-0.64^{\phantom{*}}_{\pm  1.06 }}$&$\phantom{-}\textcolor{gray}{0.03^{\phantom{*}}_{\pm  1.09 }}$&$-1.07^*_{\pm  1.04}$&$\textcolor{gray}{-0.16^{\phantom{*}}_{\pm  1.08 }}$&$-1.90^*_{\pm  1.47}$&$\textcolor{gray}{-1.22^{\phantom{*}}_{\pm  1.69 }}$&$-3.34^*_{\pm  1.30}$&$-2.89^*_{\pm  1.42}$&$-3.03^*_{\pm  1.19}$\\
 \textsc{Consequences} &$\phantom{-}10.56^*_{\pm  1.81}$&$\textcolor{gray}{-1.31^{\phantom{*}}_{\pm  1.60 }}$&$\phantom{-}9.73^*_{\pm  1.79}$&$\phantom{-}10.63^*_{\pm  1.80}$&$-5.62^*_{\pm  2.17}$&$-6.05^*_{\pm  2.33}$&$-8.71^*_{\pm  1.94}$&$-8.27^*_{\pm  2.07}$&$\phantom{-}8.81^*_{\pm  2.44}$\\
 \textsc{Conflict} &$\textcolor{gray}{-0.27^{\phantom{*}}_{\pm  1.10 }}$&$-2.02^*_{\pm  1.02}$&$\phantom{-}1.74^*_{\pm  1.17}$&$\phantom{-}\textcolor{gray}{0.92^{\phantom{*}}_{\pm  1.14 }}$&$-3.83^*_{\pm  1.27}$&$-4.67^*_{\pm  1.24}$&$-3.66^*_{\pm  1.29}$&$-3.12^*_{\pm  1.43}$&$-2.55^*_{\pm  1.26}$ \\
 \textsc{Strength} &$\phantom{-}18.63^*_{\pm  1.75}$&$\phantom{-}14.54^*_{\pm  1.69}$&$\phantom{-}8.94^*_{\pm  1.60}$&$\phantom{-}5.48^*_{\pm  1.53}$&$\phantom{-}55.84^*_{\pm  3.00}$&$\phantom{-}41.81^*_{\pm  3.51}$&$\phantom{-}22.44^*_{\pm  3.00}$&$\phantom{-}25.11^*_{\pm  3.25}$&$-5.59^*_{\pm  1.51}$\\
 \midrule
\multicolumn{10}{c}{\textsc{\textbf{Questions on}}} \\
\midrule
 \textsc{Experiences} &$-18.07^*_{\pm  2.10}$&$-16.07^*_{\pm  2.11}$&$\phantom{-}\textcolor{gray}{1.24^{\phantom{*}}_{\pm  2.21 }}$&$-7.18^*_{\pm  2.18}$&$-21.51^*_{\pm  3.00}$&$-26.92^*_{\pm  3.05}$&$-14.26^*_{\pm  3.18}$&$-12.41^*_{\pm  3.40}$&$-7.46^*_{\pm  2.88}$ \\
 \textsc{Perspectives} &$\phantom{-}1.06^*_{\pm  0.92}$&$-2.10^*_{\pm  0.74}$&$\phantom{-}2.41^*_{\pm  0.97}$&$\phantom{-}1.37^*_{\pm  0.93}$&$-1.59^*_{\pm  1.10}$&$-3.15^*_{\pm  0.88}$&$\phantom{-}\textcolor{gray}{1.30^{\phantom{*}}_{\pm  1.47 }}$&$\phantom{-}\textcolor{gray}{0.03^{\phantom{*}}_{\pm  1.40 }}$&$-2.31^*_{\pm  0.88}$\\
 \textsc{Emotions} &$-9.92^*_{\pm  1.11}$&$-10.44^*_{\pm  1.08}$&$-3.91^*_{\pm  1.32}$&$-1.97^*_{\pm  1.38}$&$-11.12^*_{\pm  1.17}$&$-10.80^*_{\pm  1.27}$&$-8.87^*_{\pm  1.46}$&$-6.80^*_{\pm  1.75}$&$-2.58^*_{\pm  1.77}$\\
 \midrule
\multicolumn{10}{c}{\textsc{\textbf{Solutions}}} \\
\midrule
 \textsc{Problem-Solving} &$\phantom{-}32.16^*_{\pm  2.00}$&$\phantom{-}22.06^*_{\pm  1.96}$&$\phantom{-}16.11^*_{\pm  1.92}$&$\phantom{-}8.84^*_{\pm  1.85}$&$\phantom{-}13.81^*_{\pm  3.07}$&$\phantom{-}23.59^*_{\pm  3.55}$&$\phantom{-}31.24^*_{\pm  3.24}$&$\phantom{-}13.20^*_{\pm  3.23}$&$\phantom{-}9.20^*_{\pm  2.54}$\\
 \textsc{Planning} &$\phantom{-}19.46^*_{\pm  1.80}$&$\phantom{-}15.28^*_{\pm  1.74}$&$\phantom{-}10.47^*_{\pm  1.67}$&$\phantom{-}8.12^*_{\pm  1.63}$&$\phantom{-}30.85^*_{\pm  3.15}$&$\phantom{-}31.51^*_{\pm  3.50}$&$\phantom{-}39.46^*_{\pm  3.17}$&$\phantom{-}24.63^*_{\pm  3.27}$ & $\phantom{-}\textcolor{gray}{1.09^{\phantom{*}}_{\pm  1.99 }}$\\
 \midrule
 \multicolumn{10}{c}{\textsc{\textbf{Normalizing}}} \\
 \midrule
 \textsc{Normalizing} &$\phantom{-}9.63^*_{\pm  1.72}$&$\phantom{-}6.71^*_{\pm  1.67}$&$-3.61^*_{\pm  1.44}$&$\phantom{-}\textcolor{gray}{0.71^{\phantom{*}}_{\pm 1.55 }}$&$\phantom{-}37.69^*_{\pm  3.20}$&$\phantom{-}36.36^*_{\pm  3.54}$&$\phantom{-}2.53^*_{\pm  2.47}$&$\phantom{-}9.53^*_{\pm  2.93}$&$\phantom{-}5.15^*_{\pm  2.24}$ \\
 \midrule
 \multicolumn{10}{c}{\textsc{\textbf{Psychoeducation}}} \\
 \midrule
 \textsc{Psychoeducation}  &$\phantom{-}3.44^*_{\pm  1.06}$&$\phantom{-}13.67^*_{\pm  1.36}$&$\textcolor{gray}{-0.25^{\phantom{*}}_{\pm  0.89 }}$&$\textcolor{gray}{-0.63^{\phantom{*}}_{\pm  0.87 }}$&$\phantom{-}3.40^*_{\pm  1.73}$&$\phantom{-}3.95^*_{\pm  1.97}$&$\phantom{-}12.45^*_{\pm  2.33}$&$\phantom{-}6.10^*_{\pm  2.07}$&$\phantom{-}3.72^*_{\pm  1.50}$\\
    \bottomrule
    \end{tabular}
    }
 % \tim{why use occurrence if we could use frequency here for simplicity}
     % \tim{we need to help people interpret these values as much as possible (for all figures/tables). Here, "difference in freq" sounds like 16 means that LLM does sth 16 more times in one conv compared to good human. However, you also say average percentage difference later. clarify/simplify/unify. again wouldd this better be a figure. or can we color numbers to show high values. Clarify whether 16 means 16\% or 16x.}
    \label{tab:high_low_distribution}
    % \vspace{-10pt}
\end{table*}

==> tables/table-4-hope-distribution.tex <==
\begin{table*}[t]
    \centering
    \small
     \caption{Difference between the frequency of conversational behaviors observed in LLM therapists (GPT-4, GPT-3.5-turbo, Llama2-70b, Llama2-13b) or low-quality human therapists and the frequency of the behavior observed in high-quality human therapists based on the two conversation simulation methods (single response and full conversation) on the HOPE dataset from \cite{malhotra2022speaker}. We report the average percentage differences across the simulated conversations with standard deviations as subscripts. Positive values indicate significantly higher observed frequency of a particular behavior whereas negative values indicate significantly lower observed frequency of a particular behavior as compared to high-quality human therapists. Values in \textcolor{gray}{gray} are not statistically significant at p = 0.05 using Two-sided Student t-test. For instance, GPT-4 model with single response simulation method has $25.33\%$ more exhibited \textsc{Reflection on Needs} behavior than high-quality human therapy.}
    \resizebox{1.01\textwidth}{!}{%
    \def\arraystretch{1.15}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|ccccccccc}
         \toprule %\\[5pt]
         \multirow{2}{*}{\textbf{Behavior}} & \multicolumn{4}{c}{\textbf{LLM Single Response}} & \multicolumn{4}{c}{\textbf{LLM Full Conversation}} & \textbf{Human} \\
         \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule{10-10}
        & GPT-4 & GPT-3.5 & Llama2-70b & Llama2-13b  & GPT-4 & GPT-3.5 & Llama2-70b & Llama2-13b & Low-Quality \\
         \midrule
 \multicolumn{10}{c}{\textsc{\textbf{Reflections on}}} \\
 \midrule
 \textsc{Needs} &$\phantom{-}25.33^*_{\pm  1.54}$&$\phantom{-}17.69^*_{\pm  1.50}$&$\phantom{-}14.32^*_{\pm  1.47}$&$\phantom{-}13.94^*_{\pm  1.46}$&$\phantom{-}16.88^*_{\pm  2.52}$&$\phantom{-}22.95^*_{\pm  3.18}$&$\phantom{-}2.98^*_{\pm  2.35}$&$\phantom{-}2.94^*_{\pm  2.44}$&$-5.59^*_{\pm  2.45}$ \\
 \textsc{Emotions} &$\phantom{-}11.97^*_{\pm  1.40}$&$\phantom{-}12.68^*_{\pm  1.41}$&$\phantom{-}4.12^*_{\pm  1.30}$&$\phantom{-}7.86^*_{\pm  1.35}$&$-4.50^*_{\pm  1.73}$&$\textcolor{gray}{-1.03^{\phantom{*}}_{\pm  2.30 }}$&$-4.51^*_{\pm  1.86}$&$\phantom{-}\textcolor{gray}{1.62^{\phantom{*}}_{\pm  2.27 }}$&$-8.31^*_{\pm  1.65}$ \\
 \textsc{Values} &$\phantom{-}1.39^*_{\pm  0.65}$&$\phantom{-}\textcolor{gray}{0.50^{\phantom{*}}_{\pm  0.61 }}$&$\phantom{-}1.07^*_{\pm  0.64}$&$\phantom{-}1.40^*_{\pm  0.65}$&$\phantom{-}2.24^*_{\pm  1.18}$&$\phantom{-}1.47^*_{\pm  1.35}$&$\textcolor{gray}{-0.30^{\phantom{*}}_{\pm  0.97 }}$&$\phantom{-}\textcolor{gray}{0.10^{\phantom{*}}_{\pm  1.06 }}$&$-3.03^*_{\pm  1.19}$\\
 \textsc{Consequences} &$\phantom{-}6.54^*_{\pm  1.44}$&$\phantom{-}4.33^*_{\pm  1.42}$&$\phantom{-}3.41^*_{\pm  1.40}$&$\phantom{-}4.63^*_{\pm  1.41}$&$-7.82^*_{\pm  1.80}$&$-7.39^*_{\pm  2.17}$&$-12.70^*_{\pm  1.58}$&$-10.68^*_{\pm  1.79}$&$\phantom{-}8.81^*_{\pm  2.44}$\\
 \textsc{Conflict}&$-0.85^*_{\pm  0.76}$&$-1.64^*_{\pm  0.73}$&$\phantom{-}1.02^*_{\pm  0.82}$&$\phantom{-}1.18^*_{\pm  0.82}$&$-3.65^*_{\pm  0.85}$&$-3.86^*_{\pm  0.95}$&$-3.09^*_{\pm  0.98}$&$-1.97^*_{\pm  1.17}$&$-2.55^*_{\pm  1.26}$ \\
 \textsc{Strength} &$\phantom{-}17.38^*_{\pm  1.20}$&$\phantom{-}16.10^*_{\pm  1.18}$&$\phantom{-}6.35^*_{\pm  1.00}$&$\phantom{-}5.99^*_{\pm  0.99}$&$\phantom{-}63.18^*_{\pm  2.37}$&$\phantom{-}48.70^*_{\pm  3.15}$&$\phantom{-}28.16^*_{\pm  2.65}$&$\phantom{-}24.58^*_{\pm  2.68}$&$-5.59^*_{\pm  1.51}$ \\
 \midrule
\multicolumn{10}{c}{\textsc{\textbf{Questions on}}} \\
\midrule
 \textsc{Experiences} &$-20.01^*_{\pm  1.71}$&$-25.97^*_{\pm  1.68}$&$\phantom{-}2.37^*_{\pm  1.74}$&$\phantom{-}\textcolor{gray}{0.54^{\phantom{*}}_{\pm  1.74 }}$&$-29.07^*_{\pm  2.52}$&$-38.42^*_{\pm  2.65}$&$-19.36^*_{\pm  2.90}$&$-17.16^*_{\pm  3.03}$&$-7.46^*_{\pm  2.88}$\\
 \textsc{Perspectives} &$\phantom{-}1.13^*_{\pm  0.84}$&$-2.25^*_{\pm  0.72}$&$\phantom{-}5.18^*_{\pm  0.95}$&$\phantom{-}4.11^*_{\pm  0.92}$&$-3.20^*_{\pm  0.94}$&$-4.75^*_{\pm  0.80}$&$\textcolor{gray}{-1.03^{\phantom{*}}_{\pm  1.27 }}$&$-1.57^*_{\pm  1.25}$&$-2.31^*_{\pm  0.88}$\\
 \textsc{Emotions} &$-7.52^*_{\pm  0.85}$&$-5.18^*_{\pm  0.93}$&$\phantom{-}1.26^*_{\pm  1.09}$&$\phantom{-}5.03^*_{\pm  1.16}$&$-9.46^*_{\pm  0.87}$&$-8.56^*_{\pm  1.11}$&$-7.37^*_{\pm  1.18}$&$-1.97^*_{\pm  1.74}$&$-2.58^*_{\pm  1.77}$\\
 \midrule
\multicolumn{10}{c}{\textsc{\textbf{Solutions}}} \\
\midrule
 \textsc{Problem-Solving} &$\phantom{-}33.04^*_{\pm  1.46}$&$\phantom{-}38.61^*_{\pm  1.47}$&$\phantom{-}13.30^*_{\pm  1.32}$&$\phantom{-}5.14^*_{\pm  1.20}$&$\phantom{-}16.93^*_{\pm  2.37}$&$\phantom{-}30.41^*_{\pm  3.16}$&$\phantom{-}35.56^*_{\pm  2.83}$&$\phantom{-}17.79^*_{\pm  2.69}$&$\phantom{-}9.20^*_{\pm  2.54}$\\
 \textsc{Planning} &$\phantom{-}13.48^*_{\pm  1.29}$&$\phantom{-}18.48^*_{\pm  1.34}$&$\phantom{-}6.49^*_{\pm  1.18}$&$\phantom{-}4.62^*_{\pm  1.14}$&$\phantom{-}32.68^*_{\pm  2.57}$&$\phantom{-}30.17^*_{\pm  3.13}$&$\phantom{-}42.27^*_{\pm  2.82}$&$\phantom{-}22.36^*_{\pm  2.76}$&$\phantom{-}\textcolor{gray}{1.09^{\phantom{*}}_{\pm  1.99 }}$ \\
 \midrule
 \multicolumn{10}{c}{\textsc{\textbf{Normalizing}}} \\
 \midrule
 \textsc{Normalizing}&$\phantom{-}12.21^*_{\pm  1.31}$&$\phantom{-}16.45^*_{\pm  1.36}$&$-1.78^*_{\pm  1.07}$&$\phantom{-}\textcolor{gray}{0.86^{\phantom{*}}_{\pm  1.12 }}$&$\phantom{-}38.13^*_{\pm  2.61}$&$\phantom{-}35.73^*_{\pm  3.20}$&$\phantom{-}5.44^*_{\pm  2.18}$&$\phantom{-}5.98^*_{\pm  2.29}$&$\phantom{-}5.15^*_{\pm  2.24}$ \\
 \midrule
 \multicolumn{10}{c}{\textsc{\textbf{Psychoeducation}}} \\
 \midrule
 \textsc{Psychoeducation} &$\phantom{-}5.75^*_{\pm  0.81}$&$\phantom{-}5.07^*_{\pm  0.78}$&$\phantom{-}2.67^*_{\pm  0.69}$&$\phantom{-}\textcolor{gray}{0.18^{\phantom{*}}_{\pm  0.58 }}$&$\phantom{-}4.32^*_{\pm  1.34}$&$\phantom{-}6.36^*_{\pm  1.84}$&$\phantom{-}16.16^*_{\pm  2.18}$&$\phantom{-}7.35^*_{\pm  1.77}$&$\phantom{-}3.72^*_{\pm  1.50}$\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:hope_distribution}
    % \vspace{-10pt}
\end{table*}




% \begin{table*}[t]
%     \centering
%     \small
%     \resizebox{0.99\textwidth}{!}{%
%     \def\arraystretch{1.15}
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{l|ccccccccc}
%          \toprule %\\[5pt]
%          \multirow{2}{*}{\textbf{Behavior}} & \multicolumn{4}{c}{\textbf{LLM Single Response}} & \multicolumn{4}{c}{\textbf{LLM Full Conversation}} & \textbf{Human} \\
%          \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule{10-10}
%         & GPT-4 & GPT-3.5-Turbo & Llama2-70b & Llama2-13b  & GPT-4 & GPT-3.5-Turbo & Llama2-70b & Llama2-13b & Low-Quality \\
%          \midrule
%  \multicolumn{10}{c}{\textbf{Reflections on}} \\
%  \midrule
%  Needs & & & & & & & & & \\
%  Emotions & & & & & & & & & \\
%  Values & & & & & & & & & \\
%  Consequences & & & & & & & & & \\
%  Conflict & & & & & & & & & \\
%  \midrule
% \multicolumn{10}{c}{\textbf{Questions on}} \\
% \midrule
%  Experiences & & & & & & & & & \\
%  Perspectives & & & & & & & & & \\
%  Emotions & & & & & & & & & \\
%  \midrule
% \multicolumn{10}{c}{\textbf{Solutions}} \\
% \midrule
%  Problem-Solving & & & & & & & & & \\
%  Planning & & & & & & & & & \\
%  \midrule
%  \multicolumn{10}{c}{\textbf{Normalizing}} \\
%  \midrule
%  Normalizing & & & & & & & & & \\
%  \midrule
%  \multicolumn{10}{c}{\textbf{Psychoeducation}} \\
%  \midrule
%  Psychoeducation  & & & & & & & & & \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{HOPE Dataset}
%     \label{tab:hope_distribution}
%     % \vspace{-10pt}
% \end{table*}

==> tables/table-5-high-low-liwc.tex <==

\begin{table*}[t]
    \centering
    \small
    \caption{Difference between the word usage of LIWC categories in LLM therapists (GPT-4, GPT-3.5-turbo, Llama2-70b, Llama2-13b) or low-quality human therapists and the word usage of LIWC categories in high-quality human therapists average for simulations with reference of High-Low Quality dataset.
    We report the average percentage differences across the simulated conversations with standard deviations as subscripts. Positive values indicate significantly higher observed frequency whereas negative values indicate significantly lower observed frequency of a particular LIWC category as compared to high-quality human therapists. Values in \textcolor{gray}{gray} are not statistically significant at p = 0.05 using Two-sided Student t-test. For instance, GPT-4 responses contain $0.227\%$ more Positive Emotion words than high-quality human therapy.  
    }
    \resizebox{0.8\textwidth}{!}{%
    \def\arraystretch{1.15}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|ccccc}
         \toprule %\\[5pt]
         \multirow{2}{*}{\textbf{Word Attribute}} & \multicolumn{4}{c}{\textbf{LLM Simulated Response}}  & \textbf{Human} \\
         \cmidrule(lr){2-5} \cmidrule(lr){6-6} 
        & GPT-4 & GPT-3.5 & Llama2-70b & Llama2-13b & Low-Quality \\
         \midrule
 \multicolumn{6}{c}{\textbf{Emotion (LIWC)}} \\
 \midrule
    Positive Emotion&$\phantom{-}0.227_{0.076}$&$\phantom{-}\textcolor{gray}{0.018_{0.074}}$&$-0.172_{0.080}$&$\textcolor{gray}{-0.063_{0.084}}$&$\phantom{-}0.448_{0.103}$\\
 Negative Emotion &$\phantom{-}\textcolor{gray}{0.017_{0.058}}$&$\phantom{-}0.281_{0.059}$&$\phantom{-}0.165_{0.060}$&$\textcolor{gray}{-0.077_{0.060}}$&$\phantom{-}\textcolor{gray}{0.046_{0.113}}$\\
 Stress &$\phantom{-}\textcolor{gray}{0.044_{0.057}}$&$\phantom{-}0.344_{0.058}$&$\phantom{-}0.383_{0.060}$&$\phantom{-}\textcolor{gray}{0.045_{0.060}}$&$\phantom{-}\textcolor{gray}{0.119_{0.114}}$\\
 Sadness &$\phantom{-}0.328_{0.031}$&$\phantom{-}0.484_{0.032}$&$\phantom{-}0.348_{0.032}$&$\phantom{-}0.228_{0.034}$&$\phantom{-}0.378_{0.052}$\\
Sympathy&$\phantom{-}0.096_{0.020}$&$\phantom{-}0.196_{0.022}$&$\phantom{-}0.158_{0.023}$&$\phantom{-}0.119_{0.023}$&$\phantom{-}0.334_{0.033}$\\
\midrule
\multicolumn{6}{c}{\textbf{Wellbeing (LIWC)}} \\
\midrule
 Meaning &$\phantom{-}2.054_{0.064}$&$\phantom{-}1.692_{0.063}$&$\phantom{-}0.791_{0.064}$&$\phantom{-}0.514_{0.067}$&$\phantom{-}1.567_{0.109}$\\
 Purpose &$\phantom{-}2.320_{0.067}$&$\phantom{-}2.020_{0.067}$&$\phantom{-}1.060_{0.067}$&$\phantom{-}0.721_{0.071}$&$\phantom{-}1.877_{0.115}$\\
 Motivation &$\phantom{-}2.054_{0.063}$&$\phantom{-}1.836_{0.063}$&$\phantom{-}0.882_{0.061}$&$\phantom{-}0.642_{0.066}$&$\phantom{-}1.750_{0.105}$\\
   \midrule
\multicolumn{6}{c}{\textbf{Wellness (LIWC)}} \\
\midrule
 Health &$\phantom{-}1.493_{0.066}$&$\phantom{-}1.628_{0.070}$&$\phantom{-}0.765_{0.064}$&$\phantom{-}0.392_{0.074}$&$\phantom{-}1.124_{0.182}$\\
 Wellness &$\phantom{-}0.720_{0.030}$&$\phantom{-}0.605_{0.031}$&$\phantom{-}0.371_{0.027}$&$\phantom{-}0.252_{0.036}$&$\phantom{-}0.498_{0.098}$\\
  \midrule
\multicolumn{6}{c}{\textbf{Behavioral Activation (LIWC)}} \\
\midrule
  Behavioral Activation &$\phantom{-}3.267_{0.111}$&$\phantom{-}2.650_{0.114}$&$\phantom{-}2.334_{0.118}$&$\phantom{-}1.718_{0.125}$&$\phantom{-}2.282_{0.179}$\\
 \midrule
\multicolumn{6}{c}{\textbf{Focus (LIWC)}} \\
\midrule
Self &$-0.906_{0.080}$&$-0.795_{0.081}$&$-1.270_{0.079}$&$-0.737_{0.083}$&$-1.440_{0.172}$\\
Other &$\phantom{-}\textcolor{gray}{0.035_{0.120}}$&$-0.429_{0.121}$&$-1.312_{0.128}$&$-2.062_{0.131}$&$-1.109_{0.208}$\\
\midrule
\multicolumn{6}{c}{\textbf{Other (LIWC)}} \\
\midrule
  BigWords&$\phantom{-}13.529_{0.188}$&$\phantom{-}12.012_{0.192}$&$\phantom{-}13.869_{0.223}$&$\phantom{-}9.536_{0.245}$&$\phantom{-}12.936_{0.332}$\\
         \bottomrule
    \end{tabular}
    }
    

    \label{tab:high-low-liwc}
    % \vspace{-10pt}
\end{table*}



==> tables/table-6-hope-liwc.tex <==

\begin{table*}[t]
    \centering
    \small
        \caption{Difference between the word usage of LIWC categories in LLM therapists (GPT-4, GPT-3.5-turbo, Llama2-70b, Llama2-13b) or low-quality human therapists and the word usage of LIWC categories in high-quality human therapists on average for simulations with the reference of HOPE dataset.
    We report the average percentage differences across the simulated conversations with standard deviations as subscripts. Positive values indicate significantly higher observed frequency whereas negative values indicate significantly lower observed frequency of a particular LIWC category as compared to high-quality human therapists. Values in \textcolor{gray}{gray} are not statistically significant at p = 0.05  using Two-sided Student t-test. For instance, GPT-4 responses with $0.617\%$ Positive Emotion than high-quality human therapy.}
    \resizebox{0.8\textwidth}{!}{%
    \def\arraystretch{1.15}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|ccccc}
         \toprule %\\[5pt]
         \multirow{2}{*}{\textbf{Word Attribute}} & \multicolumn{4}{c}{\textbf{LLM Simulated Response}}  & \textbf{Human} \\
         \cmidrule(lr){2-5} \cmidrule(lr){6-6} 
        & GPT-4 & GPT-3.5 & Llama2-70b & Llama2-13b & Low-Quality \\
         \midrule
 \multicolumn{6}{c}{\textbf{Emotion (LIWC)}} \\
 \midrule
    Positive Emotion&$\phantom{-}0.617_{0.055}$&$\phantom{-}0.269_{0.054}$&$\phantom{-}0.110_{0.055}$&$\phantom{-}0.177_{0.057}$&$\phantom{-}0.448_{0.103}$\\
 Negative Emotion &$-0.195_{0.064}$&$\textcolor{gray}{-0.059_{0.065}}$&$\textcolor{gray}{-0.104_{0.067}}$&$-0.256_{0.067}$&$\phantom{-}\textcolor{gray}{0.046_{0.113}}$\\
 Stress &$-0.430_{0.073}$&$-0.245_{0.073}$&$-0.162_{0.076}$&$-0.344_{0.076}$&$\phantom{-}\textcolor{gray}{0.119_{0.114}}$\\
 Sadness &$\phantom{-}0.273_{0.044}$&$\phantom{-}0.366_{0.046}$&$\phantom{-}0.152_{0.046}$&$\phantom{-}0.166_{0.047}$&$\phantom{-}0.378_{0.052}$\\
Sympathy&$\phantom{-}0.075_{0.021}$&$\phantom{-}0.148_{0.024}$&$\phantom{-}0.089_{0.023}$&$\phantom{-}0.150_{0.025}$&$\phantom{-}0.334_{0.033}$\\
\midrule
\multicolumn{6}{c}{\textbf{Wellbeing (LIWC)}} \\
\midrule
 Meaning &$\phantom{-}2.300_{0.054}$&$\phantom{-}1.863_{0.054}$&$\phantom{-}0.894_{0.056}$&$\phantom{-}0.680_{0.055}$&$\phantom{-}1.567_{0.109}$\\
 Purpose &$\phantom{-}2.518_{0.055}$&$\phantom{-}2.257_{0.057}$&$\phantom{-}1.027_{0.057}$&$\phantom{-}0.830_{0.059}$&$\phantom{-}1.877_{0.115}$\\
 Motivation &$\phantom{-}2.387_{0.048}$&$\phantom{-}2.251_{0.051}$&$\phantom{-}0.972_{0.048}$&$\phantom{-}0.859_{0.052}$&$\phantom{-}1.750_{0.105}$\\
   \midrule
\multicolumn{6}{c}{\textbf{Wellness (LIWC)}} \\
\midrule
 Health &$\phantom{-}0.729_{0.067}$&$\phantom{-}0.862_{0.069}$&$\phantom{-}0.172_{0.069}$&$\phantom{-}\textcolor{gray}{0.021_{0.069}}$&$\phantom{-}1.124_{0.182}$\\
 Wellness &$\phantom{-}0.660_{0.019}$&$\phantom{-}0.489_{0.020}$&$\phantom{-}0.232_{0.015}$&$\phantom{-}0.209_{0.017}$&$\phantom{-}0.498_{0.098}$\\
  \midrule
\multicolumn{6}{c}{\textbf{Behavioral Activation (LIWC)}} \\
\midrule
  Behavioral Activation &$\phantom{-}2.831_{0.093}$&$\phantom{-}2.567_{0.097}$&$\phantom{-}1.645_{0.096}$&$\phantom{-}1.325_{0.102}$&$\phantom{-}2.282_{0.179}$\\
 \midrule
\multicolumn{6}{c}{\textbf{Focus (LIWC)}} \\
\midrule
Self &$-0.497_{0.057}$&$-0.228_{0.060}$&$-0.636_{0.060}$&$-0.628_{0.060}$&$-1.440_{0.172}$\\
Other&$\textcolor{gray}{-0.133_{0.106}}$&$-0.670_{0.108}$&$-1.519_{0.112}$&$-2.039_{0.114}$&$-1.109_{0.208}$\\
\midrule
\multicolumn{6}{c}{\textbf{Other (LIWC)}} \\
\midrule
  BigWords&$\phantom{-}11.612_{0.176}$&$\phantom{-}7.906_{0.180}$&$\phantom{-}10.714_{0.203}$&$\phantom{-}7.946_{0.209}$&$\phantom{-}12.936_{0.332}$\\
         \bottomrule
    \end{tabular}
    }

    \label{tab:hope-liwc}
    % \vspace{-10pt}
\end{table*}


==> tables/table-9-all-liwc.tex <==

\begin{table*}[t]
    \centering
    \small
    \caption{Difference between the word usage of LIWC categories in LLM therapists (GPT-4, GPT-3.5-turbo, Llama2-70b, Llama2-13b) or low-quality human therapists and the word usage of LIWC categories in high-quality human therapists on average.
    We report the absolute average percentage differences across the simulated conversations with standard deviations as subscripts. Values $>0$ indicate significantly higher observed frequency  whereas values $<0$ indicate significantly lower observed frequency of particular word attribute as compared to high-quality human therapy. Values in \textcolor{gray}{gray} are not statistically significantly different from zero at p = 0.05 using Two-sided Student t-test. For instance, GPT-4 responds with 12.593\% more BigWords than high-quality human therapy. We find that all LLM therapists use significantly more BigWords than low-quality human therapy.
    }
    \resizebox{0.8\textwidth}{!}{%
    \def\arraystretch{1.15}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|ccccc}
         \toprule %\\[5pt]
         \multirow{2}{*}{\textbf{Word Attribute}} & \multicolumn{4}{c}{\textbf{LLM Simulated Response}}  & \textbf{Human} \\
         \cmidrule(lr){2-5} \cmidrule(lr){6-6} 
        & GPT-4 & GPT-3.5 & Llama2-70b & Llama2-13b & Low-Quality \\
         \midrule
 \multicolumn{6}{c}{\textbf{Emotion (LIWC)}} \\
 \midrule
    Positive Emotion&$\phantom{-}0.508_{0.042}$&$\phantom{-}0.211_{0.040}$&$\phantom{-}\textcolor{gray}{0.052_{0.043}}$&$\phantom{-}0.114_{0.045}$&$\phantom{-}0.448_{0.103}$\\
 Negative Emotion &$\textcolor{gray}{-0.054_{0.043}}$&$\phantom{-}\textcolor{gray}{0.073_{0.043}}$&$\phantom{-}\textcolor{gray}{0.000_{0.044}}$&$-0.180_{0.044}$&$\phantom{-}\textcolor{gray}{0.046_{0.113}}$\\
 Stress &$-0.182_{0.047}$&$\phantom{-}\textcolor{gray}{0.002_{0.047}}$&$\phantom{-}\textcolor{gray}{0.060_{0.048}}$&$-0.172_{0.048}$&$\phantom{-}\textcolor{gray}{0.119_{0.114}}$\\
 Sadness &$\phantom{-}0.334_{0.027}$&$\phantom{-}0.409_{0.028}$&$\phantom{-}0.232_{0.028}$&$\phantom{-}0.184_{0.029}$&$\phantom{-}0.378_{0.052}$\\
Sympathy&$\phantom{-}0.096_{0.014}$&$\phantom{-}0.187_{0.015}$&$\phantom{-}0.123_{0.015}$&$\phantom{-}0.133_{0.016}$&$\phantom{-}0.334_{0.033}$\\
\midrule
\multicolumn{6}{c}{\textbf{Wellbeing (LIWC)}} \\
\midrule
 Meaning &$\phantom{-}2.201_{0.039}$&$\phantom{-}1.770_{0.038}$&$\phantom{-}0.805_{0.039}$&$\phantom{-}0.579_{0.040}$&$\phantom{-}1.567_{0.109}$\\
 Purpose &$\phantom{-}2.429_{0.041}$&$\phantom{-}2.130_{0.041}$&$\phantom{-}1.001_{0.041}$&$\phantom{-}0.758_{0.042}$&$\phantom{-}1.877_{0.115}$\\
 Motivation &$\phantom{-}2.236_{0.037}$&$\phantom{-}2.048_{0.037}$&$\phantom{-}0.906_{0.036}$&$\phantom{-}0.740_{0.038}$&$\phantom{-}1.750_{0.105}$\\
   \midrule
\multicolumn{6}{c}{\textbf{Wellness (LIWC)}} \\
\midrule
 Health &$\phantom{-}0.862_{0.048}$&$\phantom{-}1.141_{0.050}$&$\phantom{-}0.312_{0.049}$&$\phantom{-}\textcolor{gray}{0.069_{0.051}}$&$\phantom{-}1.124_{0.182}$\\
 Wellness &$\phantom{-}0.648_{0.020}$&$\phantom{-}0.528_{0.020}$&$\phantom{-}0.264_{0.018}$&$\phantom{-}0.199_{0.020}$&$\phantom{-}0.498_{0.098}$\\
  \midrule
\multicolumn{6}{c}{\textbf{Behavioral Activation (LIWC)}} \\
\midrule
  Behavioral Activation &$\phantom{-}3.055_{0.068}$&$\phantom{-}2.575_{0.069}$&$\phantom{-}1.984_{0.071}$&$\phantom{-}1.534_{0.074}$&$\phantom{-}2.282_{0.179}$\\
 \midrule
\multicolumn{6}{c}{\textbf{Focus (LIWC)}} \\
\midrule
Self &$-0.862_{0.047}$&$-0.587_{0.048}$&$-1.029_{0.047}$&$-0.790_{0.049}$&$-1.440_{0.172}$\\
Other &$\textcolor{gray}{-0.103_{0.075}}$&$-0.645_{0.075}$&$-1.435_{0.080}$&$-2.062_{0.081}$&$-1.109_{0.208}$\\
\midrule
\multicolumn{6}{c}{\textbf{Other (LIWC)}} \\
\midrule
  BigWords&$\phantom{-}12.593_{0.123}$&$\phantom{-}9.937_{0.124}$&$\phantom{-}11.708_{0.141}$&$\phantom{-}8.446_{0.148}$&$\phantom{-}12.936_{0.332}$\\
         \bottomrule
    \end{tabular}
    }

    % \vspace{-10pt}
    \label{tab:all-liwc}
    % \vspace{-10pt}
\end{table*}


==> tables/tables_old.tex <==
\begin{table*}[t]
    \centering
    \small
    \resizebox{1.2\textwidth}{!}{%
    \def\arraystretch{1.15}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|cccccccccc}
         \toprule %\\[5pt]
         \multirow{2}{*}{\textbf{Conversational Behavior}} & \multicolumn{5}{c}{\textbf{Single Response}} & \multicolumn{5}{c}{\textbf{Full Conversation}} \\
         \cmidrule(lr){2-6} \cmidrule(lr){7-11} 
        & GPT-4 & GPT-3.5-Turbo & Llama2-70b & Guanaco-65b & Vicuna-33b & GPT-4 & GPT-3.5-Turbo & Llama2-70b & Guanaco-65b & Vicuna-33b     \\
         \midrule
 \multicolumn{11}{c}{\textbf{Reflections}} \\
 \midrule
 Makes Needs Explicit&$\textcolor{gray}{-0.38_{1.94 }}$&$\phantom{-}\textcolor{gray}{1.36_{1.96 }}$&$\phantom{-}8.29_{2.03}$&$-2.79_{1.92}$&$\textcolor{gray}{-1.20_{1.93 }}$&$\phantom{-}20.90_{6.42}$&$\phantom{-}\textcolor{gray}{0.59_{3.18 }}$&$\phantom{-}\textcolor{gray}{1.19_{2.53 }}$&&
 \\
 Makes Emotions Explicit &$\phantom{-}5.63_{1.68}$&$\phantom{-}6.17_{1.69}$&$\phantom{-}\textcolor{gray}{1.20_{1.59 }}$&$-2.33_{1.52}$&$\phantom{-}\textcolor{gray}{0.33_{1.57 }}$&$\phantom{-}8.30_{5.41}$&$-3.58_{2.32}$&$-7.92_{1.63}$&&\\
 Makes Values Explicit &$-1.25_{1.03}$&$\textcolor{gray}{-0.51_{1.06 }}$&$-1.23_{1.03}$&$-2.60_{0.97}$&$-2.51_{0.98}$&$\textcolor{gray}{-0.93_{3.03 }}$&$-3.72_{1.31}$&$-3.74_{1.09}$&&\\
 Makes Consequences Explicit &$-6.76_{1.46}$&$-4.43_{1.52}$&$\phantom{-}8.11_{1.76}$&$\phantom{-}2.18_{1.67}$&$\phantom{-}4.45_{1.71}$&$\phantom{-}6.97_{5.42}$&$-6.98_{2.18}$&$-7.30_{1.77}$&& \\
 Makes Conflict Explicit &$\textcolor{gray}{-0.64_{1.08 }}$&$-1.77_{1.03}$&$\phantom{-}1.84_{1.17}$&$-1.36_{1.05}$&$\textcolor{gray}{-0.87_{1.07 }}$&$\textcolor{gray}{-1.16_{3.04 }}$&$-3.74_{1.35}$&$-4.39_{1.06}$&&\\
 \midrule
\multicolumn{11}{c}{\textbf{Questions}} \\
\midrule
 Evokes Concrete Elaboration &$\textcolor{gray}{-1.66_{2.20 }}$&$\textcolor{gray}{-0.87_{2.20 }}$&$-3.15_{2.20}$&$\phantom{-}5.11_{2.22}$&$-7.04_{2.18}$&$-25.69_{5.24}$&$-21.34_{3.17}$&$-20.04_{2.59}$&&\\
 Evokes Perspective Elaboration &$\phantom{-}\textcolor{gray}{0.90_{0.90 }}$&$-1.79_{0.76}$&$\phantom{-}2.28_{0.97}$&$\phantom{-}\textcolor{gray}{0.81_{0.90 }}$&$\phantom{-}1.07_{0.91}$&$\phantom{-}\textcolor{gray}{0.30_{2.69 }}$&$-2.66_{0.97}$&$\phantom{-}\textcolor{gray}{0.99_{1.20 }}$&&\\
 Emotions Check-in&$-8.91_{1.15}$&$-9.21_{1.14}$&$-3.74_{1.33}$&$-2.00_{1.38}$&$-3.40_{1.34}$&$-7.29_{2.92}$&$-8.71_{1.54}$&$-6.13_{1.51}$&&\\
 \midrule
\multicolumn{11}{c}{\textbf{Solutions}} \\
\midrule
 Problem-Solving&$\phantom{-}17.05_{1.93}$&$\phantom{-}18.94_{1.94}$&$\phantom{-}10.37_{1.87}$&$\phantom{-}10.68_{1.88}$&$\phantom{-}5.89_{1.81}$&$\phantom{-}27.77_{6.38}$&$\phantom{-}24.91_{3.43}$&$\phantom{-}25.77_{2.66}$&&\\
 Planning&$\phantom{-}13.67_{1.72}$&$\phantom{-}14.08_{1.72}$&$\phantom{-}7.78_{1.62}$&$\phantom{-}6.82_{1.61}$&$\phantom{-}5.81_{1.58}$&$\phantom{-}17.35_{5.83}$&$\phantom{-}29.62_{3.35}$&$\phantom{-}34.63_{2.59}$&& \\
 \midrule
 \multicolumn{11}{c}{\textbf{Normalizing}} \\
 \midrule
 Normalizing &$\textcolor{gray}{-0.44_{1.52 }}$&$-1.82_{1.49}$&$\textcolor{gray}{-1.13_{1.50 }}$&$-2.24_{1.48}$&$\phantom{-}4.43_{1.62}$&$\phantom{-}14.10_{5.74}$&$\phantom{-}31.42_{3.40}$&$\phantom{-}10.59_{2.32}$&&\\
 \midrule
 \multicolumn{11}{c}{\textbf{Teaching}} \\
 \midrule
 Psychoeducation &$\phantom{-}3.28_{1.05}$&$\phantom{-}6.58_{1.17}$&$-0.90_{0.85}$&$\phantom{-}1.67_{0.98}$&$\textcolor{gray}{-0.69_{0.87 }}$&$\textcolor{gray}{-0.52_{2.58 }}$&$\phantom{-}4.91_{1.98}$&$\phantom{-}4.43_{1.49}$&&\\
 \midrule
 \multicolumn{11}{c}{\textbf{Emotion (LIWC)}} \\
 \midrule
    Positive Emotion &$\phantom{-}\textcolor{gray}{0.07_{0.00}}$&$\textcolor{gray}{-0.08_{0.00}}$&$\textcolor{gray}{-0.07_{0.01}}$&$-0.210_{0.005}$&$\textcolor{gray}{-0.12_{0.01}}$&$\phantom{-}0.366_{0.007}$&$\phantom{-}0.391_{0.005}$&$\phantom{-}0.376_{0.004}$&&
 \\
 Negative Emotion &$-0.174_{0.004}$&$-0.112_{0.004}$&$-0.320_{0.004}$&$\textcolor{gray}{-0.40_{0.00}}$&$\textcolor{gray}{-0.37_{0.00}}$&$\textcolor{gray}{-0.42_{0.01}}$&$\textcolor{gray}{-0.53_{0.00}}$&$-0.713_{0.004}$&&\\
 Stress &$\phantom{-}0.231_{0.004}$&$\phantom{-}0.285_{0.004}$&$\phantom{-}0.180_{0.004}$&$\phantom{-}0.072_{0.004}$&$\phantom{-}0.080_{0.005}$&$\textcolor{gray}{-0.02_{0.01}}$&$\textcolor{gray}{-0.25_{0.00}}$&$-0.304_{0.004}$&& \\
 Sadness  &$-0.358_{0.004}$&$-0.312_{0.004}$&$-0.610_{0.004}$&$-0.710_{0.004}$&$-0.581_{0.004}$&$-0.426_{0.006}$&$-0.708_{0.004}$&$-0.826_{0.004}$&& \\
 Sympathy&$-0.823_{0.004}$&$-0.786_{0.004}$&$-0.976_{0.004}$&$-0.945_{0.004}$&$-0.930_{0.004}$&$-0.827_{0.005}$&$\textcolor{gray}{-1.02_{0.00}}$&$-0.995_{0.004}$&& \\
\midrule
\multicolumn{11}{c}{\textbf{Wellbeing (LIWC)}} \\
\midrule
 Meaning &$\phantom{-}1.065_{0.004}$&$\phantom{-}1.519_{0.004}$&$\phantom{-}0.579_{0.004}$&$\phantom{-}0.697_{0.004}$&$\phantom{-}0.728_{0.005}$&$\phantom{-}1.803_{0.008}$&$\phantom{-}1.709_{0.005}$&$\phantom{-}0.828_{0.004}$&&\\
 Purpose &$\phantom{-}1.192_{0.004}$&$\phantom{-}1.695_{0.004}$&$\phantom{-}0.783_{0.004}$&$\phantom{-}0.904_{0.005}$&$\phantom{-}0.813_{0.005}$&$\phantom{-}2.097_{0.009}$&$\phantom{-}2.479_{0.006}$&$\phantom{-}1.393_{0.005}$&& \\
 Motivation &$\phantom{-}0.800_{0.004}$&$\phantom{-}1.309_{0.004}$&$\phantom{-}0.475_{0.004}$&$\phantom{-}0.566_{0.005}$&$\phantom{-}0.476_{0.005}$&$\phantom{-}1.707_{0.008}$&$\phantom{-}2.124_{0.006}$&$\phantom{-}0.967_{0.004}$&& \\
 Health &$\phantom{-}0.646_{0.004}$&$\phantom{-}1.348_{0.005}$&$\phantom{-}0.268_{0.004}$&$\phantom{-}0.486_{0.005}$&$\phantom{-}0.243_{0.005}$&$\phantom{-}1.743_{0.011}$&$\phantom{-}1.936_{0.007}$&$\phantom{-}0.315_{0.004}$&& \\
 Wellness &$-0.765_{0.004}$&$-0.584_{0.004}$&$-0.889_{0.004}$&$-0.868_{0.004}$&$-0.905_{0.004}$&$-0.426_{0.006}$&$-0.258_{0.005}$&$-0.567_{0.004}$&& \\
  Behavioral Activation &$\phantom{-}3.678_{0.005}$&$\phantom{-}3.927_{0.005}$&$\phantom{-}3.333_{0.006}$&$\phantom{-}3.546_{0.006}$&$\phantom{-}3.422_{0.007}$&$\phantom{-}5.009_{0.012}$&$\phantom{-}6.467_{0.009}$&$\phantom{-}5.985_{0.007}$&&\\
 \midrule
\multicolumn{11}{c}{\textbf{Focus (LIWC)}} \\
\midrule
Self &$\phantom{-}0.756_{0.004}$&$\phantom{-}0.760_{0.004}$&$\phantom{-}0.644_{0.005}$&$\phantom{-}0.606_{0.005}$&$\phantom{-}0.420_{0.005}$&$\phantom{-}0.452_{0.007}$&$\phantom{-}\textcolor{gray}{1.17_{0.01}}$&$\phantom{-}0.163_{0.005}$&& \\
Other &$\phantom{-}7.741_{0.005}$&$\phantom{-}7.728_{0.005}$&$\phantom{-}5.928_{0.006}$&$\phantom{-}5.836_{0.006}$&$\phantom{-}5.659_{0.007}$&$\phantom{-}6.611_{0.011}$&$\phantom{-}\textcolor{gray}{7.72_{0.01}}$&$\phantom{-}5.012_{0.006}$&& \\
\midrule
\multicolumn{11}{c}{\textbf{Other (LIWC)}} \\
\midrule
  BigWords &$\phantom{-}19.401_{0.007}$&$\phantom{-}19.368_{0.007}$&$\phantom{-}16.898_{0.010}$&$\phantom{-}18.561_{0.013}$&$\phantom{-}17.084_{0.012}$&$\phantom{-}25.407_{0.025}$&$\phantom{-}21.993_{0.013}$&$\phantom{-}30.745_{0.016}$&& \\
         \bottomrule
    \end{tabular}
    }
    \caption{Comparison of conversational behaviors between human and model (human $-$ model). We report the average percentage differences across conversations in dataset with standard deviations as subscripts. For LIWC, we report the average differences. The number with grey color is statistical insignificant ($p > 0.05$).  }
    \vspace{-10pt}
\end{table*}

\begin{table*}[t]
    \centering
    \small
    \resizebox{1.2\textwidth}{!}{%
    \def\arraystretch{1.15}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|cccccccccc}
         \toprule %\\[5pt]
         \multirow{2}{*}{\textbf{Conversational Behavior}} & \multicolumn{5}{c}{\textbf{Single Response}} & \multicolumn{5}{c}{\textbf{Full Conversation}} \\
         \cmidrule(lr){2-6} \cmidrule(lr){7-11} 
        & GPT-4 & GPT-3.5-Turbo & Llama2-70b & Guanaco-65b & Vicuna-33b & GPT-4 & GPT-3.5-Turbo & Llama2-70b & Guanaco-65b & Vicuna-33b     \\
         \midrule
 \multicolumn{11}{c}{\textbf{Reflections}} \\
 \midrule
 Makes Needs Explicit&$\textcolor{gray}{-0.38_{1.94 }}$&$\phantom{-}\textcolor{gray}{1.36_{1.96 }}$&$\phantom{-}8.29_{2.03}$&$-2.79_{1.92}$&$\textcolor{gray}{-1.20_{1.93 }}$&$\phantom{-}20.90_{6.42}$&$\phantom{-}\textcolor{gray}{0.59_{3.18 }}$&$\phantom{-}\textcolor{gray}{1.19_{2.53 }}$&&


 \\
 Makes Emotions Explicit &$\phantom{-}5.63_{1.68}$&$\phantom{-}6.17_{1.69}$&$\phantom{-}\textcolor{gray}{1.20_{1.59 }}$&$-2.33_{1.52}$&$\phantom{-}\textcolor{gray}{0.33_{1.57 }}$&$\phantom{-}8.30_{5.41}$&$-3.58_{2.32}$&$-7.92_{1.63}$&&\\
 Makes Values Explicit &$-1.25_{1.03}$&$\textcolor{gray}{-0.51_{1.06 }}$&$-1.23_{1.03}$&$-2.60_{0.97}$&$-2.51_{0.98}$&$\textcolor{gray}{-0.93_{3.03 }}$&$-3.72_{1.31}$&$-3.74_{1.09}$&&\\
 Makes Consequences Explicit &$-6.76_{1.46}$&$-4.43_{1.52}$&$\phantom{-}8.11_{1.76}$&$\phantom{-}2.18_{1.67}$&$\phantom{-}4.45_{1.71}$&$\phantom{-}6.97_{5.42}$&$-6.98_{2.18}$&$-7.30_{1.77}$&& \\
 Makes Conflict Explicit &$\textcolor{gray}{-0.64_{1.08 }}$&$-1.77_{1.03}$&$\phantom{-}1.84_{1.17}$&$-1.36_{1.05}$&$\textcolor{gray}{-0.87_{1.07 }}$&$\textcolor{gray}{-1.16_{3.04 }}$&$-3.74_{1.35}$&$-4.39_{1.06}$&&\\
 \midrule
\multicolumn{11}{c}{\textbf{Questions}} \\
\midrule
 Evokes Concrete Elaboration &$\textcolor{gray}{-1.66_{2.20 }}$&$\textcolor{gray}{-0.87_{2.20 }}$&$-3.15_{2.20}$&$\phantom{-}5.11_{2.22}$&$-7.04_{2.18}$&$-25.69_{5.24}$&$-21.34_{3.17}$&$-20.04_{2.59}$&&\\
 Evokes Perspective Elaboration &$\phantom{-}\textcolor{gray}{0.90_{0.90 }}$&$-1.79_{0.76}$&$\phantom{-}2.28_{0.97}$&$\phantom{-}\textcolor{gray}{0.81_{0.90 }}$&$\phantom{-}1.07_{0.91}$&$\phantom{-}\textcolor{gray}{0.30_{2.69 }}$&$-2.66_{0.97}$&$\phantom{-}\textcolor{gray}{0.99_{1.20 }}$&&\\
 Emotions Check-in&$-8.91_{1.15}$&$-9.21_{1.14}$&$-3.74_{1.33}$&$-2.00_{1.38}$&$-3.40_{1.34}$&$-7.29_{2.92}$&$-8.71_{1.54}$&$-6.13_{1.51}$&&\\
 \midrule
\multicolumn{11}{c}{\textbf{Solutions}} \\
\midrule
 Problem-Solving&$\phantom{-}17.05_{1.93}$&$\phantom{-}18.94_{1.94}$&$\phantom{-}10.37_{1.87}$&$\phantom{-}10.68_{1.88}$&$\phantom{-}5.89_{1.81}$&$\phantom{-}27.77_{6.38}$&$\phantom{-}24.91_{3.43}$&$\phantom{-}25.77_{2.66}$&&\\
 Planning&$\phantom{-}13.67_{1.72}$&$\phantom{-}14.08_{1.72}$&$\phantom{-}7.78_{1.62}$&$\phantom{-}6.82_{1.61}$&$\phantom{-}5.81_{1.58}$&$\phantom{-}17.35_{5.83}$&$\phantom{-}29.62_{3.35}$&$\phantom{-}34.63_{2.59}$&& \\
 \midrule
 \multicolumn{11}{c}{\textbf{Normalizing}} \\
 \midrule
 Normalizing &$\textcolor{gray}{-0.44_{1.52 }}$&$-1.82_{1.49}$&$\textcolor{gray}{-1.13_{1.50 }}$&$-2.24_{1.48}$&$\phantom{-}4.43_{1.62}$&$\phantom{-}14.10_{5.74}$&$\phantom{-}31.42_{3.40}$&$\phantom{-}10.59_{2.32}$&&\\
 \midrule
 \multicolumn{11}{c}{\textbf{Teaching}} \\
 \midrule
 Psychoeducation &$\phantom{-}3.28_{1.05}$&$\phantom{-}6.58_{1.17}$&$-0.90_{0.85}$&$\phantom{-}1.67_{0.98}$&$\textcolor{gray}{-0.69_{0.87 }}$&$\textcolor{gray}{-0.52_{2.58 }}$&$\phantom{-}4.91_{1.98}$&$\phantom{-}4.43_{1.49}$&&\\

    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of conversational behaviors between human and model (human $-$ model). We report the average percentage differences across conversations in dataset with standard deviations as subscripts. The number with grey color is statistical insignificant ($p > 0.05$).  }
    \vspace{-10pt}
\end{table*}


\begin{table*}[t]
    \centering
    \small
    \resizebox{1.2\textwidth}{!}{%
    \def\arraystretch{1.15}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|cccc|cccc|c}
         \toprule %\\[5pt]
         \multirow{2}{*}{\textbf{Conversational Behavior}} & \multicolumn{4}{c}{\textbf{Single Response}} & \multicolumn{4}{c}{\textbf{Full Conversation}} \\
         \cmidrule(lr){2-5} \cmidrule(lr){6-9} 
        & GPT-4 & GPT-3.5-Turbo & Llama2-70b & Llama2-13b  & GPT-4 & GPT-3.5-Turbo & Llama2-70b & Llama2-13b & Low-Quality \\
         \midrule
 \multicolumn{11}{c}{\textbf{Emotion (LIWC)}} \\
 \midrule
    Positive Emotion &$\phantom{-}\textcolor{gray}{0.07_{0.00}}$&$\textcolor{gray}{-0.08_{0.00}}$&$\textcolor{gray}{-0.07_{0.01}}$&$-0.210_{0.005}$&$\textcolor{gray}{-0.12_{0.01}}$&$\phantom{-}0.366_{0.007}$&$\phantom{-}0.391_{0.005}$&$\phantom{-}0.376_{0.004}$&&
 \\
 Negative Emotion &$-0.174_{0.004}$&$-0.112_{0.004}$&$-0.320_{0.004}$&$\textcolor{gray}{-0.40_{0.00}}$&$\textcolor{gray}{-0.37_{0.00}}$&$\textcolor{gray}{-0.42_{0.01}}$&$\textcolor{gray}{-0.53_{0.00}}$&$-0.713_{0.004}$&&\\
 Stress &$\phantom{-}0.231_{0.004}$&$\phantom{-}0.285_{0.004}$&$\phantom{-}0.180_{0.004}$&$\phantom{-}0.072_{0.004}$&$\phantom{-}0.080_{0.005}$&$\textcolor{gray}{-0.02_{0.01}}$&$\textcolor{gray}{-0.25_{0.00}}$&$-0.304_{0.004}$&& \\
 Sadness  &$-0.358_{0.004}$&$-0.312_{0.004}$&$-0.610_{0.004}$&$-0.710_{0.004}$&$-0.581_{0.004}$&$-0.426_{0.006}$&$-0.708_{0.004}$&$-0.826_{0.004}$&& \\
 Sympathy&$-0.823_{0.004}$&$-0.786_{0.004}$&$-0.976_{0.004}$&$-0.945_{0.004}$&$-0.930_{0.004}$&$-0.827_{0.005}$&$\textcolor{gray}{-1.02_{0.00}}$&$-0.995_{0.004}$&& \\
\midrule
\multicolumn{11}{c}{\textbf{Wellbeing (LIWC)}} \\
\midrule
 Meaning &$\phantom{-}1.065_{0.004}$&$\phantom{-}1.519_{0.004}$&$\phantom{-}0.579_{0.004}$&$\phantom{-}0.697_{0.004}$&$\phantom{-}0.728_{0.005}$&$\phantom{-}1.803_{0.008}$&$\phantom{-}1.709_{0.005}$&$\phantom{-}0.828_{0.004}$&&\\
 Purpose &$\phantom{-}1.192_{0.004}$&$\phantom{-}1.695_{0.004}$&$\phantom{-}0.783_{0.004}$&$\phantom{-}0.904_{0.005}$&$\phantom{-}0.813_{0.005}$&$\phantom{-}2.097_{0.009}$&$\phantom{-}2.479_{0.006}$&$\phantom{-}1.393_{0.005}$&& \\
 Motivation &$\phantom{-}0.800_{0.004}$&$\phantom{-}1.309_{0.004}$&$\phantom{-}0.475_{0.004}$&$\phantom{-}0.566_{0.005}$&$\phantom{-}0.476_{0.005}$&$\phantom{-}1.707_{0.008}$&$\phantom{-}2.124_{0.006}$&$\phantom{-}0.967_{0.004}$&& \\
 Health &$\phantom{-}0.646_{0.004}$&$\phantom{-}1.348_{0.005}$&$\phantom{-}0.268_{0.004}$&$\phantom{-}0.486_{0.005}$&$\phantom{-}0.243_{0.005}$&$\phantom{-}1.743_{0.011}$&$\phantom{-}1.936_{0.007}$&$\phantom{-}0.315_{0.004}$&& \\
 Wellness &$-0.765_{0.004}$&$-0.584_{0.004}$&$-0.889_{0.004}$&$-0.868_{0.004}$&$-0.905_{0.004}$&$-0.426_{0.006}$&$-0.258_{0.005}$&$-0.567_{0.004}$&& \\
  Behavioral Activation &$\phantom{-}3.678_{0.005}$&$\phantom{-}3.927_{0.005}$&$\phantom{-}3.333_{0.006}$&$\phantom{-}3.546_{0.006}$&$\phantom{-}3.422_{0.007}$&$\phantom{-}5.009_{0.012}$&$\phantom{-}6.467_{0.009}$&$\phantom{-}5.985_{0.007}$&&\\
 \midrule
\multicolumn{11}{c}{\textbf{Focus (LIWC)}} \\
\midrule
Self &$\phantom{-}0.756_{0.004}$&$\phantom{-}0.760_{0.004}$&$\phantom{-}0.644_{0.005}$&$\phantom{-}0.606_{0.005}$&$\phantom{-}0.420_{0.005}$&$\phantom{-}0.452_{0.007}$&$\phantom{-}\textcolor{gray}{1.17_{0.01}}$&$\phantom{-}0.163_{0.005}$&& \\
Other &$\phantom{-}7.741_{0.005}$&$\phantom{-}7.728_{0.005}$&$\phantom{-}5.928_{0.006}$&$\phantom{-}5.836_{0.006}$&$\phantom{-}5.659_{0.007}$&$\phantom{-}6.611_{0.011}$&$\phantom{-}\textcolor{gray}{7.72_{0.01}}$&$\phantom{-}5.012_{0.006}$&& \\
\midrule
\multicolumn{11}{c}{\textbf{Other (LIWC)}} \\
\midrule
  BigWords &$\phantom{-}19.401_{0.007}$&$\phantom{-}19.368_{0.007}$&$\phantom{-}16.898_{0.010}$&$\phantom{-}18.561_{0.013}$&$\phantom{-}17.084_{0.012}$&$\phantom{-}25.407_{0.025}$&$\phantom{-}21.993_{0.013}$&$\phantom{-}30.745_{0.016}$&& \\
         \bottomrule
    \end{tabular}
    }
    \caption{Comparison of conversational behaviors between human and model (human $-$ model). We report the average percentile differences across conversations in dataset with standard deviations as subscripts. The number with grey color is statistical insignificant ($p > 0.05$).  }
    \vspace{-10pt}
\end{table*}


\begin{table*}[h!]
\resizebox{\textwidth}{!}{%
\def\arraystretch{1.15}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{c|cccccc}\toprule
 Role&Method&Classification&Model/Prompt& Macro-Precision & Macro-Recall & \textbf{Macro-F1}\\ \midrule
 % \multicolumn{2}{c}{Retrieval}& Random& 9.6 & \textbf{3.6} & 8.4 \\
 % && SBERT& \textbf{15.2} & 1.9 & \textbf{12.8} \\[1.5mm] \hline
 
  \multirow{6}{*}{Therapist}& \multirow{2}{*}{\thead{Finetune\\ (GPT-3)}} & Multi-label& Text-davinci & $51.6_{3.2}$ & $47.9_{3.7}$ & $49.6_{2.8}$ \\[1.5mm] 
 && Multi-label & Gpt-3.5 turbo  & $45.9_{3.7}$ & $31.1_{3.1}$ & $37.1_{3.4}$  \\[1.5mm] \cline{2-7} \noalign{\vspace{0.8ex}}
 & \multirow{3}{*}{\thead{\\Prompting\\ (GPT-4)}} & Multi-label & Definitions  & $45.4_{1.9}$ & $57.8_{3.8}$ & $50.8_{1.9}$  \\[1.5mm]
  & & Multi-label & Definitions \& Examples  & $56.0_{1.7}$ & $59.5_{3.7}$ & $\textbf{57.7}_{\textbf{2.5}}$  \\[1.5mm]
  & & Binary label & Definitions \& Examples  & $49.4_{2.6}$ & $52.2_{2.1}$ & $50.7_{1.8}$  \\[1.5mm] \cline{2-7} \noalign{\vspace{0.8ex}}
  & \multicolumn{3}{c}{\textit{Random baseline}}  & \textit{11.8}_{\textit{0.7}}& \textit{17.6}_{\textit{2.9}} & \textit{14.1}_{\textit{1.3}}  \\  \hline
  \midrule
    \multirow{5}{*}{Client}& \thead{Finetune\\ (GPT-3)} & Multi-label& Text-davinci & $45.2_{5.9}$ & $36.8_{6.0}$ & $40.4_{5.2}$ \\[1.5mm]  \cline{2-7} \noalign{\vspace{0.8ex}}
 & \multirow{3}{*}{\thead{\\Prompting\\ (GPT-4)}} & Multi-label & Definitions  & $65.6_{7.3}$ & $81.6_{7.5}$ & $72.6_{6.8}$  \\[1.5mm]
  & & Multi-label & Definitions \& Examples  & $72.6_{6.7}$ & $76.4_{10.2}$ & $74.4_{8.4}$  \\[1.5mm]
  & & Binary label & Definitions \& Examples  & $73.4_{5.9}$ & $80.3_{7.2}$ & $\textbf{76.7}_{\textbf{6.3}}$  \\[1.5mm] \cline{2-7} \noalign{\vspace{0.8ex}}
  & \multicolumn{3}{c}{\textit{Random baseline}}  & \textit{23.2}_{\textit{5.1}}& \textit{29.6}_{\textit{8.0}} & \textit{25.9}_{\textit{6.2}}  \\

 
\bottomrule 
\end{tabular}
}
\caption{Classification models performance of conversational behaviors on Therapist and Client. We present the metrics in \% with different methods (finetune, prompting)}
\end{table*}
